Introduction to Variational Quantum Algorithms

This document is a pdf version of the series of blogposts about variational quantum algorithms (VQA) I originally posted on my blog Musty Thoughts. It provides an explanation of the basic variational algorithms, such as Variational Quantum Eigensolver (VQE) and Quantum Approximate Optimization Algorithm (QAOA), as well as a more general framework for VQAs. It also describes some more advanced techniques that can be used to make these algorithms more efficient, as well as the challenges associated with using them.

==> Previous_Sections/How_they_work.tex <==
\begin{document}
Let’s just explain what a VQA is:

VQA is an algorithm which tries to find the minimum value of some function using:
\begin{itemize}
    \item A parametrized quantum circuit as one of the steps for calculating a function’s value.
    \item Classical optimization to find the optimal parameters of the circuit.
\end{itemize}

If you want to read a more detailed definition I recommend [Jhonathan Romero Fontalvo’s dissertation, section 1.2](https://dash.harvard.edu/bitstream/handle/1/42029810/ROMEROFONTALVO-DISSERTATION-2019.pdf?sequence=1&isAllowed=y)

Also, two more things just to set the expectations right:
\begin{itemize}
    \item I’ve written this assuming running the programs on an actual QPU (Quantum Processing Unit), not a simulator. Accounting for both cases made some of the diagrams harder to read and it’s pretty straightforward to imagine what changes are needed if we run it on a simulator.
    \item This is a popular article aimed at explaining the complexity of VQAs. It’s not a scientific paper and some of the choices I made might turn out to not be the most universal or 100% correct. In such cases please leave a comment, I’d love to discuss it.

\end{itemize}


With that being said, let’s get started with the 

\subsection{Basic Setup}

When I first started learning about Variational Quantum Algorithms (VQAs), I wasn’t able to appreciate how complex they are. 

In my mind, a quantum algorithm looked like this:

    
    \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/WORK/01_basic_diagram.png}
            \caption{Caption later\Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}
    
However, when I started learning and thinking more about running such algorithms on near-term quantum computers, I quickly realized this view is oversimplified; there are several crucial intermediate steps in a VQA that must be taken to make the best use of today’s devices.

One of the important questions one needs to ask is “How do I know what circuit I need to run?” The choice of the circuit is mainly motivated by the problem we want to solve and in the case of VQAs, we use so-called “Ansatz circuits” (see [VQE article]({post_url 2019-11-18-Variational-Quantum-Eigensolver-explained }) for more details). You can think about it as a circuit template – it has some parameters which correspond (directly or indirectly) to parameters of gates as well as some “hyperparameters” – e.g. the number of layers, the types of gates for a given layer, etc.

    \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/WORK/02_with_ansatz.png}
            \caption{Caption later\Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}
    
As you can see on the diagram, I’m using different colors for different blocks. Here’s what they mean:

\begin{itemize}
    \item Blue boxes are objects created/changed when we run the algorithm.
    \item Purple boxes are objects which define the problem we’re solving and algorithm's hyperparameters.
    \item Green boxes are objects which can perform some actions. They change the content of the blue boxes and the way they do it is informed by the purple ones.
    \item Backend is red, because it’s the actual quantum computer and I wanted it to stand out :)
\end{itemize}

In addition to the specific problem, the choice or design of the quantum circuit is determined by the backend/device. Devices we have available today cannot execute any quantum circuit we can imagine. The two main reasons for that are:

\begin{itemize}
    \item Implemented (or “native”) gate sets – in the classical Boolean logic, people sometimes say that the NAND gate is a “universal” gate. This means that you can construct any circuit using only NAND gates. In quantum computing, it’s slightly more complicated. From what I’ve seen, usually a set of three gates is used to construct a universal set, but there are some schemes which involve 2 gates (or as it turns out even 1 gate!) (see [wiki](https://en.wikipedia.org/wiki/Quantum_logic_gate#Universal_quantum_gates){:target="_blank"} and [here’s some more discussion](https://quantumcomputing.stackexchange.com/a/2015){:target="_blank"} on this topic). There are many different gate sets that you use for that purpose that are (at least on paper) equally good. But when you start implementing them on the real hardware, it turns out that some of these gates are easier to realize than others. So usually, when it comes to running a program on an actual quantum computer, you have only a handful of gate types available.
    \item Connectivity – in the ideal case, you assume that all the qubits are connected to each other. But in reality, this is often not the case – for example that would be infeasible for superconducting chips. Imagine having a chip where qubits are arranged in a line. Directly performing a CNOT gate on the first and last qubits is not possible, because these two qubits are not connected. 
\end{itemize}

We can overcome these device-imposed restrictions by introducing an additional step that translates an “abstract circuit” into an “executable circuit”, which is called compilation. In the diagram below, I’ve hidden the connectivity and available gate set under “QPU specs” box (since it depends on the specific backend we’re using I added a dashed line to indicate causation).

I’ve also added a new box “Execution”, to make the diagram more consistent and clear. 

   \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/WORK/03_with_compilation.png}
            \caption{Caption later\Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}
    
There’s one last step from the first picture that we haven’t talked about yet – getting measurements.

This one’s trivial, isn’t it? You just take a circuit, run it on your backend and measure the output, right?

Well, not necessarily. There are a couple of things to consider.

First, readout correction. As we mentioned before, quantum computers nowadays are imperfect machines. There’s no reason to think that these imperfections have spared the measurement process. When you measure your qubit, various errors can happen. Sometimes it’s impossible to say whether an error occurred, but sometimes we can detect its occurrence based on how the physical system has behaved. Then we can either discard such a sample or correct it. It is worth mentioning that measurement errors can be an order of magnitude higher compared with other types of errors (see [this talk](https://youtu.be/FklMpRiTeTA?t=1024){:target="_blank"}).

It is a good place to mention other types of error mitigation or error correction. In the most basic form it doesn’t need to be used for VQAs, as they are designed to be somewhat resistant to noise. While they can benefit from it (see e.g. [here](https://arxiv.org/abs/1804.06969){:target="_blank"}), I’m leaving it out from our discussion. Adding error correction is what I would consider an advanced modification of basic VQA, which is outside of the scope of this article. An additional complication is that depending on implementation it could live in different places in our diagram – e.g. ansatz or compilation.

Second, as you might remember from the VQE article, for a given Hamiltonian we need to measure each Pauli term separately, i.e. we need to run a separate circuit. However, this is the most naïve approach – in reality, there are certain grouping strategies that make it possible to measure multiple terms simultaneously. This also means that choosing a certain grouping strategy might influence how the circuit (in particular its last part) will look like.

Third, there’s a very fundamental issue of deciding how many samples (sometimes also called “shots”) you want to get. For a given problem one sample might be too little, but one million might be way more than necessary. In most cases we just decide on a particular number, e.g. 10000. But to make things even more complicated, you might want to use various numbers of shots for different groups or even change it in different iterations of the optimization loop.

So here’s what our picture looks like now:

   \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/WORK/04_with_measurements.png}
            \caption{Caption later\Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}

As you can see, I’ve also added a Hamiltonian box. It might influence how our ansatz looks like (e.g. in QAOA) or whether we need to rotate the state before measuring (in VQE), but it also guides the grouping strategy. 

So we’re getting the measurements at the end, but are they something that we really care about? Aren’t they just a means to an end? Sure they are! 
In the case of VQE we want to calculate the expectation value of some operator – for each term you take the measurements, we check what eigenvector they represent and calculate the corresponding eigenvalue (for the details please check out [the VQE article]({post_url 2019-11-18-Variational-Quantum-Eigensolver-explained })). 
For QAOA we don’t really need to do all that, we can just take the bitstring we got, plug it into the cost function and get the cost value.
As you can see, the exact thing that happens here might vary, so let’s just call this part “postprocessing” and agree that it translates all the measurements we got into “energy” or “cost value”. 

   \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/WORK/05_with_energy.png}
            \caption{Caption later\Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}
    
The picture so far can be divided into two parts. One is everything we do to generate a circuit that we’ll run on our hardware. The second one is everything we do with this circuit – how we run it, what we do with the measurements etc. 
It’s by no means a formal distinction, but I found it helpful to think about it in such a way.


That’s already quite a lot, but we’re just starting! You see, all that we have seen so far is about running a circuit for a single set of parameters. But how do we know which parameters we need to choose?

Glad that you’ve asked!

Welcome to the land of the

\subsection{Optimization Loop}

Basically, the optimization loop looks like this:

   \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/WORK/06_basic_optimizer.png}
            \caption{Caption later\Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}
We take some parameters, prepare a circuit based on that, execute and measure that, calculate the energy value and pass it to the optimizer alongside the initial parameters. Given that optimizer can actually need past values to work properly, there’s also this dashed loop around it.

The new block here is “Optimizer”, but actually we haven’t discussed “Parameters” properly yet, so let’s start from that.

Parameters…  we know the optimizer updates parameters based on the value of the cost function, but where does the first set of parameters come from? They come from some “parameter initialization” procedure. In order to initialize them, we need to actually know a couple of things:
\begin{itemize}
    \item How many parameters do we have?
    \item Are they constrained in any way?
    \item What method do we want to use for the initialization?
\end{itemize}

Answers to the first two questions depend specifically on the ansatz that we’re using and the problem we want to solve. For example in the case of QAOA our number of parameters depends solely on the number of layers and not on the problem – we just have a single pair of ($\beta$, $\gamma$) per layer. Also, since our ansatz has periodic behavior with respect to these angles, we might want to constrain them to ($0$, $2\pi$). 
There’s still the last question to answer – how to choose good initial angles? The most basic method is to just choose them at random, but there are many other methods to get better initial values and it turns out to influence the performance of the algorithm a lot –definitely more than I suspected.

So our picture looks like this now:

   \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/WORK/07_with_initialization.png}
            \caption{Caption later\Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}

We know initial parameters, we run our circuit, we get some energy value. We pass it to the optimizer and it spits out new parameters. But how does this happen?

\subsection{Optimizers - gradients}


In the process of writing, I have realized that it’s hard to talk about this topic without some basic concepts from the theory of optimization. Let’s say we have some function (we usually call it cost function), which depends on N parameters. Whenever we put these parameters into our function, it returns a single number (in some cases it might be a vector, but that’s uncommon in this context). If we calculated the values of the function for all possible sets of parameters, we would get a full optimization landscape. It’s very convenient to think about it in terms of N-dimensional space, where each set of parameters represents a point (or vector) in such space. Another useful concept is a gradient, which tells us what’s the direction and rate of the fastest increase of the function for any point.

If this sounds abstract, you can think about a map. Our function in this case will take two parameters – latitude and longitude – and return a single value: height. Global (*nomen omen*) maximum would be Mount Everest and the global minimum Mariana Trench. A steep slope means the gradient is big in that direction, a plateau means it’s small (or even zero).
You can generalize such a map to an N-dimensional space and most intuitions still hold.

In the case of the optimization problem, we usually want to find the global minimum and there are many methods to do that. For the sake of simplicity let’s start with a basic one called “gradient descent”. It works as follows:

\begin{enumerate}
    \item Select a point
    \item Calculate the value of the cost function
    \item Calculate a gradient
    \item Make a step in the direction indicated by the gradient – since we want to get to the minimum, we’re looking for the negative values of the gradient
    \item You’re at a new point, go back to 2.
    \item Finish if no further improvement is possible.
\end{enumerate}

Now we’re ready to get back to our VQAs. If we translate this algorithm into the world of VQAs it looks something like this:
\begin{enumerate}
    \item Select initial parameters
    \item Run your circuit and get the energy value.
    \item Calculate gradients.
    \item Update parameters 
    \item Go back to 2.
    \item Finish if no further improvement is possible.
\end{enumerate}

But how do you calculate gradients? Sometimes we know the exact mathematical formula, but in the case of QC that’s usually not the case. One of the most basic methods to approximate it is called “finite differences”. Let’s say we have a function of one variable $f(x)$. We can check what’s the value of the gradient by calculating its values at $f(x+\epsilon)$ and $f(x-\epsilon)$, where $\epsilon$ is just a very small number. The gradient is $g(x) = \frac{1}{2* \epsilon} (f(x+\epsilon) - f(x-\epsilon)) $. 
If we have a function with more variables, we need to check it for various combinations of $ x_i \pm \epsilon$, but the general idea stays the same.

One of the problems with calculating gradients this way is that now we have to evaluate our cost function 3 times every iteration: $f(x)$, $f(x+\epsilon)$ and $f(x-\epsilon)$. If we have more variables, we will need even more evaluations. This might mean that most of your calculations on a quantum computer actually go towards calculating gradients.

Fortunately, there are some other ways of calculating gradients which work better than this. However, some of them might require modifying your circuit. Also, there are some optimizers that don’t even use gradients, but describing all that would be way beyond the scope of this article.

his part was quite lengthy, but it illustrates a couple of points pretty well:
\begin{itemize}
    \item Notice that there’s nothing “quantum” about the optimization process we used here. In general, most (if not all) of the optimizers used in VQAs don’t really care whether they optimize parameters for quantum computers, neural networks, or a mathematical function. They just care about the input and output. 
    \item There’s actually one thing that is specific for QC (though it doesn’t necessarily apply to quantum only). We have limited precision while calculating the value of the cost function (and its gradients) on a quantum computer, associated with the finite number of measurements.
    \item It’s easy to miss some big performance issues when you just look at the big picture. For example, if we understood all the pieces of the VQA except for the optimizer we’re using, we could still end up with very bad performance due to a naive method of calculating gradient. 
    \item VQAs have some distinct qualities which make some optimizers work well and some not. For example, every calculation of the cost function is computationally expensive, since you need to use a QPU to get it. Another example is the precision issue that I've mentioned above.
\end{itemize}

\subsection{Optimizers - other aspects}
We have initial parameters, we know how to calculate gradients (or we decide to go with a gradient-free method) so what else do we need to know about the optimizer part?

The first thing is that an optimizer might have multiple hyperparameters, like how big the steps should be in a gradient method or how many iterations do we want to have. These hyperparameters might change throughout the optimization process (if you’re unfamiliar with the concept of hyperparameters, [this article](https://machinelearningmastery.com/difference-between-a-parameter-and-a-hyperparameter/){:target="_blank"} might be useful). 

Another thing, quite distinct from the optimizer’s parameters, is its constraints. In some cases we might need to put some constraints on the parameters (e.g. they all need to sum up to 1), which influences how the optimizer behaves. An example could be a problem where we know that our quantum state should have a fixed number of particles and our quantum circuit should not represent states with other numbers, even though it’s possible with the ansatz we use.

Lastly, an optimizer might actually modify some of the elements inside the “Circuit preparation/circuit execution” box, most notably the measurement strategy. The easiest example that comes to my mind is the one that I’ve already mentioned, i.e. changing the number of shots during the training. We can argue that in the first iterations when we’re exploring the optimization landscape, we might not need a lot of precision and we can save some QPU time by doing a smaller number of shots. However, once we start converging on the minimum, a small difference in parameters might have huge consequences, so we would rather get higher precision.

So this is what our picture looks like now:

   \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/WORK/08_with_gradient_01.png}
            \caption{Caption later\Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}

At the bottom, you can see the gradient calculation loop. For the sake of not overcomplicating this plot we’ll hide it inside the optimizer:

   \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/WORK/09_with_gradient_02.png}
            \caption{Caption later\Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}


This picture is quite accurate for standard versions of VQAs that you usually encounter. However, I’d like to cover two more cases here, which often show up in the literature

\subsection{Outside loops}

\subsubsection{Layer-by-layer training}
Many ansatzes (e.g. QAOA) can have multiple layers. One of the problems with many layers is that the more layers you have, the more parameters there are to optimize which means it’s harder to find the optimal values.
One of the methods that’s often used to help with that is layer-by-layer training. We first find the optimal parameters for the first layer of our ansatz. We keep them and then add another layer. We optimize the parameters for both layers and then add another.

In such a case our picture would look something like this:
   \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/WORK/10_with_lbl.png}
            \caption{Caption later\Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}

It’s pretty similar to the previous one, except that our parameter initialization strategy depends on the values we found for a smaller number of layers. Obviously, we might also want to change some other parameters like measurement strategy or optimizer hyperparameters.

\subsubsection{Adaptive circuits}
Recently (2020) there have been many propositions of algorithms which throughout the optimization modify the structure of the circuit itself, not only values of its parameters. As an example I’d like to use the [PECT algorithm](https://arxiv.org/abs/2010.00629){:target="_blank"}.

The main idea of this algorithm is that instead of optimizing all the parameters at once, we remove some of the parameters (and the corresponding gates) and optimize only a fraction of the parameters. We have two optimization loops – one selects which parameters we should select for optimization and the other finds the best values of these parameters.

Here we don’t change the structure of the circuit itself, rather just which gates we treat as “parameterizable”. However, there are other proposals as well, where we change the structure of the circuit itself. Actually, layer-by-layer can be treated as an example of such. Another one would be using genetic algorithms to find the optimal ansatz for our problem. Since the structure of the circuit “adapts” during the optimization, such algorithms are sometimes called “adaptive algorithms” (see e.g. [Adapt-VQE](https://arxiv.org/abs/1812.11173){:target="_blank"}).


\subsection{Summary}

Look at where you are:
   \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/WORK/09_with_gradient_02.png}
            \caption{Caption later\Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}
    
Look at where you started:
       \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/WORK/01_basic_diagram.png}
            \caption{Caption later\Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}

\end{document}

==> Previous_Sections/QAOA.tex <==
\begin{document}

Imagine a classroom where students are sending notes between each other. The teacher is annoyed by this and thanks to a meticulous invigilation knows exactly how many notes pass between each pair of students. The class is moving to a new room, where there is a huge gap in the middle, preventing students from sending notes to the other side. How should the teacher divide the class into two groups in order to minimize the number of notes being sent?

Or another example — in a far away kingdom, there were multiple merchants who all traded with each other. However, an evil imp wanted to impair the trade in this kingdom, so he decided to create an intrigue which would separate the merchants into two opposite factions, not trading between each other. The question was — who should be in which faction to maximize the losses?

What do both these situations have in common? They both can be described as a MaxCut problem — given a graph, find a way to divide it into two groups, such that the edges going between the two groups have the biggest possible weight.

In the first example, the nodes of the graph represent the students and the connections represent how many notes a given pair of students exchange. 
In the second example, the nodes are the merchants and the connections are the number of ducats, drachmas or talents their mutual trade is worth.

Let’s see what this graph might look like:

    \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/QAOA/01_graph.PNG}
            \caption{Caption later\Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}

and what’s the solution of this problem: 
    
    \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/QAOA/02_graph_solved.PNG}
            \caption{Caption later\Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}

\subsection{Why MaxCut?}
A small digression here: if you’ve seen your portion of graph and optimization problems, MaxCut might not be the most obvious example. However, we use it here for a few reasons:
\begin{itemize}
    \item MaxCut is the problem that the authors of [the original QAOA paper](https://arxiv.org/abs/1411.4028) solved with this algorithm.
    \item It is the most well-studied example of QAOA application in the literature (probably because of 1).
    \item Solution to MaxCut is a binary string (so just a string of 0s and 1s) and there is no problem with encoding the results.
    \item As far as I can tell, it has some neat mathematical properties (especially for k-regular graphs) which make it easier to analyze. If you’re interested, you can find more answers in [the original paper](https://arxiv.org/abs/1411.4028), as well as others papers by the same and these two talks: [talk 1](https://youtu.be/J8y0VhnISi8) and [talk 2](https://youtu.be/wJwsLkHWYMA).
\end{itemize}

\subsubsection{Why Combinatorial Optimization?}

As you might have already guessed, MaxCut is an example of a combinatorial optimization problem (I’ll abbreviate it to COP). This is a class of problems where we want to find the best solution from a finite set of solutions — it usually involves graphs or ordering some objects. Some well-known examples are the Traveling Salesman Problem or the Knapsack Problem.

The first problem with combinatorial optimization is that it is, well, combinatorial. This usually means that the number of all possible solutions grows extremely fast with the size of the problem — so called “exponential growth” or “combinatorial explosion”. Exponential means that the number of possible solutions typically depends on $a^n$ ($a$ is a constant depending on a problem and $n$ is the problem size). Combinatorial means that $n!$ is involved — which is even worse than exponential.

That’s not a problem in and of itself — in the case of continuous optimization we have to deal with an infinite number of possible solutions (since we use real numbers) and somehow we have efficient methods of doing that. The fact that we need to deal with discrete values actually makes things harder — or at least different. Many continuous functions we have to deal with in optimization are smooth — i.e. if we change $x$ just a little, the $f(x)$ also changes just a little, which is really helpful. For discrete functions, if we change only one bit of the solution from 0 to 1, we might get dramatically different results.

It’s also worth noting that many such problems are NP-hard – for those unfamiliar with this term it basically means that there are no efficient methods for solving exactly big instances of a given problem. If you're interested in details you can read on [wikipedia](https://en.wikipedia.org/wiki/NP-hardness), watch [this video](https://www.youtube.com/watch?v=YX40hbAHx3s) or read [this book](https://www.goodreads.com/book/show/400716.Introduction_to_the_Theory_of_Computation?from_search=true&from_srp=true&qid=riKxp0V42Y&rank=1). 

Since these problems are so difficult to solve, why do we bother? Because they are applicable in so many places that I won’t even try to list them here — apparently there is even [a book](https://www.goodreads.com/book/show/5248928-industrial-applications-of-combinatorial-optimization?from_search=true&from_srp=true&qid=xxJYpGVqpr&rank=1) just listing out where you can apply COPs.

\subsection{QAOA - Introduction}
QAOA is an algorithm which draws from various concepts. We’ll start with a description of QAOA and then we’ll go one by one through all the pieces needed to actually understand why it works.

Let’s say we have a cost Hamiltonian $H_C$ representing our problem (we will see how to create one in the section about Ising models). We can also construct an operator $U(H_C, \gamma) = e^{-i \gamma H_C}$.

Then, we can construct another operator: $H_B = \sum_{j=0}^n \sigma_j^x$ ($\sigma_j^x$ is a pauli X matrix) and corresponding to it $U(H_B, \beta) = e^{-i \beta H_B}$.

In QAOA we construct the state 
$| \gamma, \beta \rangle = U(H_B, \beta_p) U(H_C, \gamma_p) … U(H_B, \beta_1) U(H_C, \gamma_1) | s \rangle $
, where $p$ is usually called "number of steps" and denotes just how many times do we repeat applying $U(H_B, \beta) U(H_C, \gamma)$. $|s\rangle$ is the initial state, usually $|0...0 \rangle$ or $H | 0...0 \rangle = | +...+ \rangle$. We often call $\beta$ and $\gamma$ “angles”.

In order to find what are the values of angles which produce a reasonable state, we do exactly the same thing as we did [with VQE]({post_url 2019-11-18-Variational-Quantum-Eigensolver-explained }){:target="_blank"}. We start from some initial parameters, measure the state and update the angles to get a state closer to our solution in the next iteration. 

The first time I looked at these equations I was like: “Ok, let’s implement it and see how it works!”. But the more I’ve been learning, the more I started to ask questions such as: “What do we need $H_B$ for?”, “Why does $H_B$ have this exact form?”, “Why do we use these funny $e^{-iH}$ operators?” and, predominantly, “Why should it even work at all?”

Let’s find out the answers in the following paragraphs!

\subsection{Background: Adiabatic Quantum Computation (AQC)}
\subsubsection{What is AQC?}

Let’s say we have a quantum system described with a simple Hamiltonian $H_S$ with a known ground state. We also have another Hamiltonian $H_C$, whose ground states we want to learn. We can now construct a new Hamiltonian in the form of: $H(\alpha) = (1 - \alpha) H_S + \alpha H_C $. For $\alpha=0$ our system is described with $H_S$, for $\alpha=1$ by $H_C$. 

The adiabatic theorem states that if we start in the ground state of $H_S$ and very slowly start to increase $\alpha$ up to 1, then throughout the process the system will always stay in the ground state of $H(\alpha)$  — which means that at the end it will be in the ground state of $H_C$. It’s also worth mentioning that $\alpha$ could be an actual physical quantity.

Of course that’s not an easy thing to do and certain conditions apply, but in principle if the evolution is slow enough, we are able to find a solution to any problem if we can encode its solution in the ground state of $H_C$. We use the word “evolution” for the process of changing the quantum system by changing $\alpha$. Also, we often use $\alpha=\frac{t}{T}$, where $t$ is current time and $T$ is total or end time.

\subsubsection{Ising models}
There is one big assumption in the previous paragraph, which could easily ruin any potential usefulness of this method: “if we can encode its solution in the ground state of $H_C$.”
Well, if we don't know how to encode the problem, then AQC won’t help us. Fortunately, we know such encodings for many combinatorial optimization problems and we use “Ising models” to do that.

Imagine a chain of particles. Each particle has a spin which is either “up” or “down” (or +1 and -1) and it wants to have a different spin than its neighbours. We can write down the Hamiltonian for such system:

$ H(\sigma) = - \sum_{<i, j>} J_{ij} \sigma_i \sigma_j $

Here $\sigma_i$ is the spin of the i-th particle and by $\sigma$ we denote a string of all the spins — e.g. [-, -, +, + -, … ] — and $J_{ij}$ is the strength of the interaction between the particles. This mathematical description actually works equally well with lattices instead of chains. Also, we can change the behaviour of the system by changing the sign of $J_{ij}$ — if it's negative it behaves as described, but if it’s positive, then the particles will try to have the same spin direction.

This model maps very well on quantum computers — we just need to change $
\sigma_i$ to $\sigma_i^z$ (pauli Z operator acting on $i$-th qubit).

It turns out that we can encode many different COPs using Ising models — I won’t describe how to do that here, but you can find many examples in [this paper](https://arxiv.org/pdf/1302.5843.pdf). For our discussion it suffices to know that it is doable and that we can do that using only pauli Z operators.

\subsection{Problems with AQC}
Ok, so we can encode most problems of interest into Hamiltonians and we have a method which basically guarantees that we find a proper solution. So what’s the catch?

Well, there are a couple of them:

\begin{itemize}
    \item In order to work AQC requires to be very well isolated from the outside world — which is really hard to do in practice.
    \item It might require a very long time to run.
    \item You won’t be able to run it on a gate-based quantum computer. Well, while it is possible in principle, it would required much better hardware than we have today and doesn't seem to be practical in any foreseeable future
\end{itemize}
Basically, the harder your problem is, the more isolated your quantum system must be and the longer it has to run. 

\subsubsection{Relation to quantum annealing}
This seems like a good place to mention quantum annealing (QA) — the paradigm that Canadian company D-Wave is following. 
The main idea behind QA is the same as for AQC — start from a ground state of an easy Hamiltonian and slowly evolve your state towards the ground state of the interesting Hamiltonian. What’s the difference? QA is an imperfect implementation of AQC which trades some of AQC’s power for easier implementation. Although not everybody might agree on this since the line between what the community call AQC versus QA is very blurry, basically we can say that QA is a heuristic algorithm which:
1. Can be more flexible when it comes to the rate of change between two Hamiltonians (finite practical time which is on the order of microseconds in current devices) and 
2. Operates at finite temperature. 

This comparison leaves a lot of subtleties out, but I think it’s a good first approximation to start thinking about it. If someone would like to learn more, these two publications might shed some light: [Comparison of QAOA with QA and SA](https://arxiv.org/abs/1901.01903) and [AQC and QA: Theory and Practice](https://www.goodreads.com/book/show/23092024-adiabatic-quantum-computation-and-quantum-annealing?from_search=true&from_srp=true&qid=buAmNDqPcP&rank=1).


\subsection{Background: Quantum Mechanics}
In this section I’d like to review two ideas which come directly from basic quantum mechanics — time evolution of a quantum system and trotterization.

\subsubsection{Time evolution}
There is an operation which is quite common in quantum computing — taking an operator $A$ and creating another of the form $U_A = e^{-itA}$. But why would you do that?

Well, it comes from the Schrödinger equation:

$$ i \hbar \frac{d}{dt} | \Psi(t) \rangle = H | \Psi(t) \rangle $$

What it says is that the change (in time) of the state of a quantum system described by a time-independent Hamiltonian $H$ depends solely on the form of this Hamiltonian.

And if we solve the equation we see that this dependency is:

$$| \Psi(t) \rangle = e^{-iHt} | \Psi(0) \rangle $$

What does this tell us?
That if we take some state, $ | \Psi(0) \rangle$ and act on it (evolve it) with a Hamiltonian $$H$$ for a period of time $T$, we will get a state $ | \Psi(T)\rangle = e^{-iHT} | \Psi(0 \rangle$. 

If this sounds abstract, imagine an electron orbiting the proton (hydrogen atom again!). This system is defined solely by the interaction between these two particles and their initial states and we know how to describe the interaction in the form of a Hamiltonian. So by solving the Schrödinger equation we are able to get a formula describing the state of the system after time T. And if we do the math, we know it will look like this: 
$$ | \Psi(T) \rangle = e^{-iHT} | \Psi(0) \rangle$$

The key point to remember? Whenever you see an operator which looks like this $e^{-iHt}$, you can understand it as an evolution of the quantum system described by the Hamiltonian $H$.

Until this point we’ve made one silent assumption: we’ve assumed that the Hamiltonian we wanted to solve was time-independent. But when we take a look at the Hamiltonian we used for AQC ($H(\alpha) = (1 - \alpha) H_S + \alpha H_C $) and change $\alpha$ to $t$, we cannot pretend it’s time-independent. Depending on how complicated this time-dependency is, this might complicate the solution we’ve presented a little bit or a lot. In the latter case, the problem might be impossible to solve, so it’s reasonable to make some approximations.

\subsubsection{Trotterization}

Another concept important for understanding QAOA is “Trotterization”. Most of the time we want to find the ground state of a Hamiltonian which is too complicated for us to deal with directly — then it might be useful to approximate it. An example can be (surprise), a time-dependent Hamiltonian.

To help us grasp the idea we’ll get back to the “classical world”: imagine a curve. Let’s say this curve is described by some function. 

![full_curve](/assets/images/2020-05-04-Quantum-Approximate-Optimization-Algorithm-Explained/04_curve_full.png#center)

We can approximate it by a [piecewise linear function](https://en.wikipedia.org/wiki/Piecewise_linear_function). The more “pieces” we use, the better approximation we get:

![approximated_curve](/assets/images/2020-05-04-Quantum-Approximate-Optimization-Algorithm-Explained/05_curve_approx.png#center)

We can do the same with the time evolution of a quantum system for an operator $U(t)$ ($U(t)$ is actually a shorthand of $U(t, t_0)$, which means that we act for time $t$ starting from $t_0$). We can write $U(t, t_0) = U(t_n, t_{n-1}) U(t_{n-1}, t_{n-2}) … U(t_2, t_1), U(t_1, t_0)$ ([source](https://ocw.mit.edu/courses/nuclear-engineering/22-51-quantum-theory-of-radiation-interactions-fall-2012/lecture-notes/MIT22_51F12_Ch5.pdf)). The bigger $n$ we use, the better approximation we can get. Keep in mind that the time differences $\Delta t_i = t_{i+1} - t_i$ don’t need to be equal. 

Another approximation, particularly useful in quantum mechanics, is called the “Suzuki-Trotter expansion” or “Trotterization” (it is somewhat similar to other expansions we use in mathematics, like a Taylor series expansion. If you’re not familiar with this concept, I recommend watching [this video by 3Blue1Brown](https://www.youtube.com/watch?v=3d6DsjIBzJ4) ).
If our Hamiltonian has the following form $e^{A+B}$, we can use the following relation:

$$ e^{A+B} = lim_{n \rightarrow \infty} (e^{\frac{A}{n}} e^{\frac{B}{n}} )^n $$

We can look at it as approximating time evolution by $A+B$ by applying alternatively $A$ and $B$ for time intervals $\frac{1}{n}$. 
Now we have all the knowledge we need to understand what’s the motivation behind QAOA.

\subsection{QAOA revisited}
AOA creates the state: 
$$ | \gamma, \beta \rangle = U(H_B, \beta_p) U(H_C, \gamma_p) … U(H_B, \beta_1) U(H_C, \gamma_1) | s \rangle$$
, where $U(H_B, \beta) = e^{-i \beta H_B}$ and $U(H_C, \gamma) = e^{-i \gamma H_C}$ and $|s\rangle$ is the starting state (we defined it before).

First, we can now see that the operators $U_B = U(H_B, \beta)$ and $U_C = U(H_C, \gamma)$ correspond to evolving the state with the Hamiltonian $H_B$ and $H_C$ for time $\beta$ and $\gamma$. 

Second, we can also see that having several layers of $U_B U_C$ looks a lot like a trotterization of $e^{(H_B+H_C)}$. It’s not “pure” trotterization, since we have different $\beta$ and $\gamma$ for each step, so it resembles the “piecewise approximation”. But approximation of what?

Third, by combining the two previous points we can see that QAOA (somewhat) mimics adiabatic evolution from the ground state of $H_B$ to the ground state of $H_C$, which encodes our solution (remember Ising models?). So answering the question in the previous paragraph – QAOA could be (given right choice of parameters) viewed as the approximation of AQC.

This still leaves a couple of important questions open:

\begin{itemize}
    \item What's the actual relation between QAOA and AQC?
    \item Why should QAOA work?
    \item Why do we actually need $H_B$?
\end{itemize}


\subsection{Relation to AQC}

QAOA is not a perfect analogy to AQC. While there are a lot of similarities, there are also significant differences.

First of all, the goal is different. In AQC our goal is to get the ground state of the Hamiltonian. In QAOA (Quantum **Approximate** Optimization Algorithm) our goal is not really to get the exact ground state. It is to get a state which has good enough overlap with the ground state, so that we get an approximate solution.

Second of all, we could choose our angles in such ways that the evolution of a state using QAOA would mimic the evolution using AQC. But we don’t do that — in QAOA we can choose angles arbitrarily (usually using some classical optimization strategy).

And lastly, there’s something that I struggled a lot to understand (honestly, I still struggle with it ;) ). In AQC we start from $H_B$ and slowly move towards $H_C$. In QAOA we actually frantically alternate between $H_B$ and $H_C$ — more on that later.

\subsubsection{Why should it work?}

In principle, if you can get an infinite number of steps and choose angles which exactly mimic the adiabatic path, you will get the right results. It reminds me of the [universal approximation theorem](https://en.wikipedia.org/wiki/Universal_approximation_theorem) for neural networks. UAT says that if you have a one-layer neural network which is big enough, it can approximate any function, so basically solve any problem. The problem is with the “big enough” part — the requirements are astronomical for relatively simple problems. That’s why we usually don’t use gargantuan one-layer networks, but rather just stack smaller layers on top of each other.
With QAOA the case is similar — in principle we could just keep increasing the number of steps and stay close to the parameters for the adiabatic path, but in practice, we choose not to. We try to solve the problem with a smaller number of steps by finding the right set of angles. 

So we have some intuitions why it should work, but to be honest, we don’t know if it will work (at least without infinite resources) — it’s an important open question. Some of the researchers (me ;) ) are optimistic, because as it was with neural networks, they had very limited practical applications until some improvements made them an extremely useful and widely used tool. But we still don’t know whether this is the case with QAOA — solving a toy problem with an algorithm is different from solving a real problem with it.

Actually, there's a quote illustrating it from a [recent paper](https://arxiv.org/abs/2004.09002) by two of the three authors of the original QAOA paper:

No one knows if a quantum computer running a quantum algorithm will be able to outperform a classical computer on a combinatorial search problem.


\subsubsection{Why is the $H_B$ is important?}
$H_C$ is easy — it corresponds to the problem that we want to solve and hence we know why it looks the way it looks. But what about $H_B$? Why do we choose it to be just $\sum_i^N \sigma_i^x$ and not something else? Why do we even need it at all?

First, it doesn’t need to be just $\sum_i^N \sigma_i^x$. We want it to be something that does not commute with $H_C$ and this choice of $H_B$ meets this requirement and is super easy to implement (after the exponentiation we get a layer of $R_x$ gates). [This discussion](https://physics.stackexchange.com/questions/9194/what-is-the-physical-meaning-of-commutation-of-two-operators) might help you better understand why commutation of operators is significant. Another way to look at it is that choice of $H_B$ changes the expressibility of our ansatz — it allows us to reach states that we would otherwise never reach (remember the robot arm from [the VQE post]({% post_url 2019-11-18-Variational-Quantum-Eigensolver-explained %})?).

Second, why do we need it at all? One part of the answer is that it is just a part of the setup that came from AQC and the way we apply it comes from Trotterization. Unfortunately it doesn’t give us a lot of intuition or reason why not to drop it altogether. 
For me it's easier to understand this problem if we look at it from the perspective of not having $H_B$ at all. So what would happen in such a case?

We would be just repetitively applying $U_C$. But once we got into a state which is the eigenstate of $H_C$ we wouldn't get any further. This is basic linear algebra — if we apply an operator to its eigenvector, it can change its length, but not direction. The same applies if we had a $H_B$ which commutes with $H_C$. So we need this intermediate step of applying $H_B$ which allows us to escape from the local minimum. How do we make sure we escape it? Well, that's where the classical optimization loop is useful – we try to find the right values of the parameters $\beta$ and $\gamma$ which make it happen.

I came up with a metaphor which might be helpful to get some more intuition. Imagine you’re in a forest full of traps and you want to find a treasure. $H_C$ allows you to feel the treasure and move towards it, while $H_B$ provides you with a set of rules on how to move to avoid the traps. Without $H_C$ you have no idea which direction to go and without $H_B$ you cannot make any moves. This metaphor definitely has some limitations, but should work for starters :)

\subsubsection{What does the circuit look like?}
Ok, so let’s take a peek at how it looks in practice. 
The simple problem that we want to solve is Maxcut on a triangular graph (see the picture below). Two edges have weight 10 and one weight has weight 1. 

    \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/QAOA/06_graph.png}
            \caption{Caption later\Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}

The correct solution to this problem is a cut which divides this graph into two groups: \{0\} and \{1, 2\}. We can encode solution into a binary string where 0 and 1 indicates in which group given node is, for example:

\begin{itemize}
    \item 001: nodes 1 & 2 are in group 0, node 0 is in group 1
    \item 110: nodes 1 & 2 are in group 1, node 0 is in group 0
\end{itemize}

As you can see, we use representation where the rightmost bit is the least significant.

The cost function for MaxCut is the sum of costs of all the individual edges. Each individual cost is equal to: $C_{ij} = \frac{1}{2} w_{ij} (1 - z_i z_j)$, where $z_i=1$ if $i-th$ node is in group 0 and $z_i=-1$ if it’s in group 1. So if they're both in the same group $C_{ij}$ is equal to 0 and it's 1 otherwise. I know such representation might not make a lot of sense at first glance, but once you start solving this problem you will see it’s reasonable. 
Now we can translate this into Hamiltonian form: $\frac{1}{2} w_{ij} (1 - \sigma_i^z \sigma_j^z)$.

So in case of our graph, the Hamiltonian of interest is equal to:

$$ H_C = \frac{1}{2} \cdot 10 \cdot (1 - \sigma_0^z \sigma_1^z) +  \frac{1}{2} \cdot 10 \cdot (1 - \sigma_0^z \sigma_2^z) +  \frac{1}{2} (1 - \sigma_1^z \sigma_2^z) $$

Then we can take care of $H_B$ — this is easy, it’s just $\sigma^x_0 + \sigma^x_1 + \sigma^x_2$. 

Now we need to build $U_C$ and $U_B$ from these and then create a circuit out of that. How?

Well, describing this procedure is beyond the scope of this blogpost. For those of you who are curious, you can find it in [this paper](https://arxiv.org/pdf/1001.3855.pdf), section 4.

I have also not done this manually, I just used code from [a qiskit tutorial](https://qiskit.org/textbook/ch-applications/qaoa.html). You can see the result below:

![circuit](/assets/images/2020-05-04-Quantum-Approximate-Optimization-Algorithm-Explained/07_circuit.png#center)

$U_1 = e^{i \frac{\lambda}{2}}  R_Z(\lambda)$
This is for $\gamma = 0.5$ and $\beta=0.3$.

This circuit consists of 4 parts:

\begin{itemize}
    \item Hadamard gates — this is just for preparing the initial state — i.e. equal superposition of all states.
    \item $U_C$ - in our graph we had 3 edges and we can see three blocks of gates here. Each consists of one two-qubit controlled $U_1$ and two single qubit $U_1$ gates. As you can see first two are parametrized with $10 \gamma$, since the weights of the corresponding edges were equal to 10. 
    \item $U_B$ - this is just a layer of $R_X$ gates parametrized with $2 \beta$
    \item Measurements
\end{itemize}

\subsection{Why is is appropriate for NISQ}
f you don’t know what the issues with NISQ devices are, I described it already in the [article about VQE]({% post_url 2019-11-18-Variational-Quantum-Eigensolver-explained %}). So here I’ll just point out why QAOA seems like a good algorithm for NISQ:

\begin{itemize}
    \item The depth of the algorithm is scalable — the more steps we want to have, the more power QAOA has. With most current devices we’re limited to 1-2 steps (which are of little practical use), but this number will get higher with better hardware. [Recently Google published results](https://arxiv.org/abs/2004.04197) for $p=3$.
    \item Similarly to VQE, QAOA is somewhat resistant to noise (which is also shown in [the same paper from Google](https://arxiv.org/abs/2004.04197))
    \item Even though I’ve described only one particular way of creating the ansatz, there’s actually some flexibility and therefore you might be able to tune the algorithm toward specific architecture. 
\end{itemize}

\subsection{Relation to VQE}
VQE and QAOA are often mentioned together. VQE is often described as an algorithm good for chemistry calculations and QAOA as good for combinatorial optimization. It’s worthwhile to understand the relation between the two.

QAOA can be viewed as a special case of VQE. In the end, the whole circuit we’ve described above is just an ansatz, parameterizable by the angles. And since the Hamiltonian contains only Z terms, we do not need to change the basis for measurements. 

There are, however, a couple of things that make QAOA different:

\begin{itemize}
    \item The form of the ansatz is limited to the alternating form we’ve already seen.
    \item We are restricted in terms of which types of Hamiltonians we can use (i.e. Ising Hamiltonians). This also means that we don’t need to do additional rotations before measurements as we did in VQE.
    \item The last (and I think the most fundamental) difference is the goal of the algorithm. In VQE we want to find the ground state energy and in order to do that we need to reproduce the ground state. In QAOA our goal is to find the solution to the problem. To do that we don’t need to find the ground state — we just need to find a state which has a high enough probability of finding the right solution.
\end{itemize}





\end{document}

==> Previous_Sections/VQE.tex <==
\begin{document}
    \Yogi{NISQ should be mentioned in the Introduction.}


    Without going too much into the details and math, I would like to explain what we can use VQE for and why it’s important. \\
    
    VQE allows us to find an upper bound of the lowest eigenvalue of a given Hamiltonian. \\
    
    Let's break it down:
    \begin{itemize}
        \item \textbf{Upper bound} — let’s say we have some quantity and we don’t know its value. For the sake of the example, let’s say it’s the level of water in a well. We know that the water surface can’t be above the edge of the well — if that was the case, the water would spill. So this is our **upper bound**. We also know that the level cannot fall below the bottom of the well — this is our **lower bound** \MS{Formatting should be bold in all ** cases}. Sometimes when we describe a physical system, it’s very hard to find the real value, but knowing the lower or upper bound can help us estimate what the value might be.\\
        
        \item \textbf{Hamiltonian} — the Hamiltonian is a matrix which describes the possible energies of a physical system. If we know the Hamiltonian, we can calculate the behaviour of the system, learn what the physical states of the system are etc. It’s a central piece of quantum mechanics.\\
        
        \item \textbf{Eigenvalue} — a given physical system can be in various states. Each state has a corresponding energy. These states are described by the eigenvectors and their energies are equal to the corresponding eigenvalues. In particular, the lowest eigenvalue corresponds to the ground state energy.\\
        
        \item \textbf{Ground state} — this is the state of the system with the lowest energy, which means it’s the "most natural" state — i.e. a given system always tend to get there, and if it is in the ground state and is left alone, it will stay there forever.\\
    \end{itemize}
    
    These ``physical systems" and ``states" may sound abstract, so let’s try an example that’s a little bit more down-to-earth. I cannot think of anything simpler than a hydrogen atom.\\


    So we have \MS{TODO: Language} a two-particle system with a proton in the center and one electron. We can describe it with a Hamiltonian. The ground state of the electron is its first orbital. In this configuration it has some energy which corresponds to the lowest eigenvalue of the Hamiltonian. If we hit it with a photon with specific energy, it can get to the excited state (any state that’s not the ground state) — described by another eigenvector and eigenvalue.\\ 


    With all that in mind, we can reformulate our statement about VQE:\\
    \MS{This formatting looks weird, I think it doesn't need the first itemize}
    
    \begin{itemize}

        \item[] \textbf{VQE can help us to estimate the energy of the ground state of a given quantum mechanical  system} with the following caveats:
        \begin{itemize}
            \item estimate by providing us an upper bound
            \item if we know the Hamiltonian of this system
        \end{itemize}
    \end{itemize}
    
    \MS{This should actually go to a footnote} To be mathematically exact: upper/lower bounds are defined for sets, not single values. So whenever I mention "upper bound of a value" I really mean ``upper bound of the one-element set containing given value". Also, I know that stating ``Hamiltonian is a matrix" might be viewed as oversimplification, but I find it a very helpful oversimplification.\\
    
    There are at least two reasons why we care about using a quantum computers to get the energy of a ground state:
    
    \begin{itemize}
        \item Knowing a ground state is useful 
        \item It’s \MS{For some reason it displays without the apostrophe} really difficult to obtain it using a classical computer
    \end{itemize}
    
    Ground state energy is fundamental in quantum chemistry. We use this value to calculate a number of other, more interesting properties of molecules, like their reaction rates, binding strengths or molecular pathways (the different ways in which a chemical reaction can occur). Many of these calculations involve several steps, so an error in the first step will introduce an error to all the subsequent steps. Therefore if one of the values we use in the first step (e.g. energy of the ground state) is closer to the reality, so will be our final result.\\
    
    \subsection{The Variational Principle}
    
    In this and the following sections I will go into more technical details of why and how VQE actually works.\\
    
    The first piece is the variational principle.\\
    
    \MS{This whole section looks weird in \LaTeX when each sentence is a separate paragraph.}
    
    Let's say we have a Hamiltonian $H$ with eigenstates and associated eigenvalues . Then the following relation holds:
    
    $$ H | \psi_{\lambda} \rangle = \lambda | \psi_{\lambda} \rangle $$
    
    which is basically a characteristic equation (eigenequation) for $H$.\\

    The problem is that we usually don't know what the eigenstate
    $| \psi_{\lambda} \rangle$ is and what's the value of the $\lambda$. So how can we get some estimate of that?\\
    
    Well, to get the energy value for given state $| \psi \rangle$, we can use following expression:
    
    $$ \langle \psi | H | \psi \rangle = E( \psi )$$
    \MS{I think it would be useful to actualy use \\eq for the equations, so it will be easier to refer to the later. I didn't do that in the blogpost cause I didn't know how.}
    
    (We usually refer to it as calculating the "expectation value" of $H$)\\
    
    If we use an eigenstate we get:
    
    $$ \langle \psi_{\lambda} | H | \psi_{\lambda} \rangle = E_{\lambda}$$
    
    For the eigenstate associated with the smallest eigenvalue we would get $E_0$ (ground state energy). It's by definition the lowest value we can get, so if we take an arbitrary state $| \psi \rangle$ with an associated energy $E_\psi$ , we know that $E_\psi \ge E_0$ . We get equality if we're lucky enough that our state is equal to the ground state.\\
    
    The method described here is known as variational method and the following relation is known as the variational principle:
    
    $$ \langle \psi_{\lambda} | H | \psi_{\lambda} \rangle >= E_0$$
    
    Our $E_\psi$ is an upper bound for the ground state energy, so exactly what we wanted. The problem is that just knowing any upper bound doesn't yield much benefit. The closer the upper bound is to the real value, the better. In principle, we could simply try all the possible states and pick the one with the lowest energy. However, this approach isn't very practical - there are way too many states to accomplish that in a reasonable amount of time. Also, most of the states will give you really bad answers, so there is no point in trying them out.\\
    
    \subsection{Ansatz}
    
    Once you start reading papers about VQE or QAOA, you’ll start noticing that people care a lot about ansatzes. I have missed the definition of ansatz when I started learning, which meant that for a long time it was something rather abstract to me, so here I will try to give you some intuition regarding this topic.\\



    The problem (as mentioned in the previous section) is that we would like to explore the space of all the possible states in a reasonable manner. We do that using parameterizable circuits — i.e. circuits which have gates with some parameters. So let’s take a simple circuit, consisting of a single RY gate as an example. It has a single parameter — rotation angle. With this simple circuit we can represent a whole spectrum of quantum states — namely $(\alpha |0\rangle + (1-\alpha)|1\rangle)) $(see figure \ref{VQE_block}).
    
    Below you can find a visualization of this family of states using a Bloch sphere. 
    
    \begin{figure}[!htp]
        \centering
        \includegraphics[scale = 0.4]{images/VQE/image1.jpg}
        \caption{Potential positions in Bloch spehere \Yogi{reference for the image?}} \MS{What reference? I created this one by myself so I don't think reference is needed. Same for others.}
        \label{fig:VQE_bloch}
    \end{figure}
    
    However, there are many states that we can’t represent — e.g. $1/√2 * ( |0⟩ +i |1⟩)$.\\
    
    \MS{This doesn't display well, there's special notation for brakets in \LaTeX though. }
    
    In order to cover this state, we need to introduce another gate, e.g. RX. And of course find the corresponding angles. RX or RX RY are examples of simple ansatzes. The situation gets more complicated when we have to deal with multiple qubits or entanglement. In general we want to have an ansatz which:
    
    \begin{itemize}
        \item Covers many states — ideally, we want it to cover the whole space of possible states.
        \item Is shallow — the more gates you use, the higher the chance of something going wrong. We’re talking about NISQ after all.
        \item Doesn’t have too many parameters — the more parameters, the harder it is to optimize.
    \end{itemize}
    
    If the description above doesn’t give you enough intuition of what it’s about, let’s try with the following metaphor. Imagine you have a robot. This a simple robot with one rigid arm that can rotate around the central point, like in the image \ref{robot_arm}:
    
        \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/VQE/image2.jpg}
            \caption{Scara robot \Yogi{reference for the image?}}
            \label{fig:robot_1}
        \end{figure}
    
    Let’s say the robot has a pen and it can draw. In this case, no matter how hard you try, the most you can get out of it is a circle. How to improve it?\\

    Well, you can add another rotating arm at the end of the first one. Now you can cover much more — a big circle empty in the middle. 
    
        \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/VQE/image3.jpg}
            \caption{Improving the robot \Yogi{reference for the image?}}
            \label{fig:robot_2}
        \end{figure}
        
    Ok, and what if I told you that actually the arms can only move in a discrete way — i.e. they always rotate by a fixed angle. If it’s small, then you can still cover most of the space. If not — well, you will get a nice pattern. Anyway, it might be beneficial to add additional arms in this imperfect scenario to cover the space better. \\
    
    Why don’t you add another 20 arms? It sounds impractical for several reasons. The more arms you add, the harder it is to construct and control them, and it’s more error-prone. By the way, you can check out [this video](https://youtu.be/-qgreAUpPwM) \MS{Should be changed to a link} to see how crazy you could get with a similar setup in theory \Yogi{Should we mention this youtube video?} \MS{Maybe in a footnote?}. Imagine what these drawings would look like if you got even a 0.1\% error in the angles for each arm.\\

    So what does it have to do with our ansatzes?\\
    Having a good robot setup will allow you to cover a lot of space and at the same time it would be relatively simple. The same is true for ansatzes. A good ansatz is one that allows you to cover many states and which has a reasonable number of parameters — so it’s easier to control and optimize.\\
    
    \subsection{Ansatz citcuit}
    
    As we all know, to do quantum computing we use quantum circuits. So what does one for VQE looks like?\\
    
    It consists of three parts:
    \begin{itemize}
        \item Ansatz
        \item Hamiltonian
        \item Measure
    \end{itemize}
    
    We know what the ansatz part is about — it prepares the state we need in order to apply variational principle. \\

    Hamiltonian — there is a limitation on what Hamiltonians we can use with VQE. We need Hamiltonians constructed as a sum of Pauli operators (X, Y, Z) and their tensor products. So for example we can have the following Hamiltonian: $XY + YZ + Z$. Or for the multi-qubit case: $$ X_1 \otimes X_2 \otimes Y_1 - Z_1 \otimes X_2 + Z_1 $$\\


    What might be surprising is the fact that we don’t actually put any of the corresponding X, Y, Z gates into the circuit. We use them to choose in which basis we want to do a measurement. \\


    Most (if not all) contemporary quantum computers perform measurements in the so-called "computational basis". What it means is that they will tell you whether your state turned out to be 0 or 1. However, that’s not the only way to go. What if we wanted to distinguish between states $|+\rangle = |0\rangle + |1 \rangle$ and $|- \rangle = |0\rangle - |1 \rangle$ ?\\
    
    Well, measuring in the computational basis you’ll get 0 and 1 with the same probabilities for both of them, so they’re indistinguishable. To see what might help we can use the Bloch sphere again. Let’s visualize both pairs of states: $|0 \rangle$ and $|1\rangle$ (red) and $|+\rangle$ and $|-\rangle$ (green).\\
    
        \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/VQE/image4.jpg}
            \caption{bloch without rotation \Yogi{reference for the image?}}
            \label{fig:bloch_original}
        \end{figure}
    
    As you can see, in both cases they are on the opposite ends of the sphere. It means that we can switch between them by performing a rotation around the Y axis by 90 degrees. This gives us a tool to distinguish between $|+ \rangle$ and $|- \rangle$ states even if we can measure only whether the state is $|0\rangle$ or $|1\rangle$. If we start from $|+\rangle$ and perform $RY(\pi/2)$ rotation (rotation around the Y axis by 90 degrees), we will end up in the $|1\rangle$ state. If we now measure it, we will always get 1. Similar for the other state. \\
    
    After rotating applying $RY(\pi/2)$ to all the states, we will get the following Bloch sphere (notice the colors switched):
    
    \begin{figure}[!htp]
            \centering
            \includegraphics[scale = 0.2]{images/VQE/image5.jpg}
            \caption{Bloch after rotation \Yogi{reference for the image?}}
            \label{fig:bloch_rotation}
    \end{figure}
    
    
    Ok, so coming back to our Hamiltonians. The first thing we need to do is divide the sum into its elements, so called "terms". Now, for each term we look at every Pauli operator and append appropriate rotations to the circuit:
    
    \begin{itemize}
        \item $RY(-\pi/2)$ if it’s X
        \item $RX(\pi/2)$ if it’s Y
        \item We do nothing if it’s Z
    \end{itemize}
    
    There’s one more caveat here: we actually don’t do it all at once — we create a separate circuit for each term. And once we’ve done this, we are ready to perform the measurements. But how exactly do these measurements relate to the variational principle we’ve mentioned earlier? Remember this equation: $\langle \psi | H | \psi \rangle = E_{\psi}$ ?\\
    
    $| \psi \rangle$ is the state created by the ansatz. Hamiltonian is composed of sums of Pauli terms, so we can separate it into individual terms and deal with them one at the time: $H = H_1 + H_2 + … + H_n$.\\
    The question at hand is how to get from here to $\langle \psi | H_i | \psi \rangle$.\\

    We can utilise the fact that $\langle \psi | H_i | \psi \rangle$ represents the expected value of $H_i$, which can be approximated by observing (measuring) the state $| \psi \rangle$ using the right basis (one corresponding to the eigenvalues of $H_i$) and averaging the results. The more times we do that, the better precision we'll get.\\
    
    One more thing about the averaging - when we do a measurement we get either 0 or 1. Taking all the 0s and 1s and averaging them would give us an expectation value of the measurements, not expectation value of the Z operator. If we look at the Z operator, we see that it has two eigenstates $| 0 \rangle$ and $|1 \rangle$ associated with eigenvalues 1 and -1 accordingly. To calculate $\langle \psi | Z | \psi \rangle$, we need to measure our circuit many times and then substitute every ``0" with ``1" and every ``1" with ``-1".\\
    
    Ok, so let’s take a look at the following example.\\

    Let’s say the Hamiltonian is: H = 2*Z + X + I (there’s only one qubit, so I'm omitting indices).
    It is represented by the following matrix:

        $$ \begin{bmatrix}
            3       & 1 \\
           1       & -1\\
        \end{bmatrix}$$
    
    We would like to learn its ground state using VQE.\\

    To begin with — we need to choose our ansatz. We don’t want to over complicate it, let’s say our ansatz will be $RY(\theta)$. This will allow us to explore the states
    $\cos(\theta) | 0 \rangle + \sin(\theta) | 1 \rangle $.\\
    
    Our Hamiltonian has three parts : $H_1 = 2*Z,  H_2 = X, H_3 = I $.\\
    
    The first part is fairly simple. As you recall, if we have a Z gate, we don’t need to add any rotation. So our circuit for the first part of the Hamiltonian will consist just of the ansatz.\\
    
    You might wonder what should we do with the "2" in front of Z? Well, we will treat it just as weight — after we do measurements and we will be calculating the energy, the results coming from $H_1$ will count twice as much as the results coming from $H_2$ or $H_3$.\\
    
    In case of $H_2$ we have one gate: X. So we simply nee to add a $RY(-\pi/2)$ gate to our circuit. $H_3$ is the easiest one of all of them — it’s just a constant factor we need to add to our calculations and we don’t need to do any measurements.\\
    
    So in this example we need two circuits to use our VQE, you can see them below:
    
    \begin{figure}[!htp]
        \centering
        \includegraphics[scale = 0.2]{images/VQE/image6.jpg}
        \caption{Circuits \Yogi{reference for the image?}}
        \label{fig:circuits}
    \end{figure}
    
    First RYs are ansatzes, and they are parametrized by theta. Second RY in the right picture is actually $RY(-\pi/2)$. The last symbol is how we depict measurement in quantum circuits. Our Hamiltonian was: $H = H_1 + H_2 + H_3 = 2*Z + X + I$.\\
    
    So if $\theta = 0$, then we will get 2 for $H_1$, 0 for $H_2$ and 1 for $H_3$. So our $\langle \psi(0) | H | \psi(0) \rangle = 3$. If $\theta=\pi$, we get 2*(-1) for $H_1$, 0 for $H_2$ and 1 for $H_3$, $ \langle \psi(\pi) | H | \psi(\pi) \rangle = -1$. Going through all the possible values of $\theta$ would be cumbersome, so I will tell you how approach the problem of finding a good value of theta in the next section.\\
    
    This example was pretty simple and you might wonder: "Ok, but how do I deal with the case, when there are more than one Pauli matrices in one term?". It turns out that whenever you start multiplying Pauli matrices, in the end you always get another Pauli matrix multiplied by some constant. So you can always simplify your term in such way, that you will end up with a single Pauli matrix.\\
    
    And what if I have more qubits? Again, we treat each term separately, perform all the rotations that we need at the end and measure all the qubits that we need.
    
    If you would like to calculate these by hand, you might find [the notes](https://drive.google.com/file/d/1yrH4\_5AeioXbi03AmP9TBspyWlEx2ydO/view?usp=sharing) by [Christoph Trybek](https://christophtrybek.github.io/) helpful. \Yogi{Should we mention this?} \MS{I think this could go to the appendix, as I think it's pretty useful to understand what's going on.}
    
    \subsection{Hybrid Approach}
    
    
    As mentioned earlier, VQE is a hybrid, quantum-classical algorithm. It means that we don’t perform all the computations on a quantum computer, we use a classical one too. So what does that look like?\\


    You remember that ansatz has a lot of parameters, right? The problem is that we don’t know which parameters are good and which ones are crappy. So, how do we learn that? Well, we treat it as a regular optimization problem.\\ 
    
    
    Usually we start from a random set of parameters — which corresponds to a random state (keep in mind it’s created using the ansatz that we use — so it’s not a "random state chosen from the set of all possible states", but a "random state chosen from the set of all possible states we can get with given ansatz"). We perform measurements, so we know the corresponding energy (we also use the term "expectation value").\\
    
    
    Then we slightly change the parameters, which corresponds to a slightly changed state. After we perform measurements, we should get a different energy value.\\ 
    
    
    If the new energy value is lower, it means that we’re moving into a good direction. So in the next iteration we will further increase those parameters that have increased and decrease those that have decreased. If the new energy value is higher, it means we need to do the opposite. Hopefully after repeating this procedure many times, we will get to a place where no matter what changes we do to the parameters, we can’t get any better — this is our minimum.\\
    
    
    The optimization strategy I described is pretty trivial and it’s good only as an example. Choosing a right optimization method for your problem might decide whether you’ll succeed or not and is pretty difficult — there are no silver bullets here. You can choose from a range of methods, like SGD (Stochastic Gradient Descent), BFGS or Nelder-Mead method.\\
    
    
    Ok, but this section was supposed to be about explaining how the hybrid quantum-classical thing works, right?\\
    
    \Yogi{You want to leave this here or move to another section?}
    \MS{I would leave it for now}
    
    So the idea is that we use a quantum computer (sometimes called QPU — quantum processing unit) for one thing only — to get the energy value for a given set of parameters. Everything else — so the whole optimization part — happens on a regular computer.\\
    
    
    To make it more tangible here’s a (probably incomplete) list.\\
    
    What a QPU does \Yogi{Have a look at this list}:
    \MS{The list was totally wrong, why noone told me that before? fixed it. }
    
    
    \begin{itemize}
        \item Given a set of parameters, returns us a set of measurements.
    \end{itemize}

    What a classical computer does:

    \begin{itemize}
        \item Given a set of measurements calculates the energy value (it’s usually some kind of averaging)
        \item Performs optimization procedure.
        \item Calculates what a new set of parameters should be
        \item Checks whether we have reached the minimum
        \item Makes sure we dont make more iterations than we should have done
    \end{itemize}
    
    \MS{Missing section title}
    
    As already mentioned, NISQ stands for “Noisy Intermediate Scale Quantum” (John Preskill explains what it exactly means in this [video](https://www.youtube.com/watch?v=h4nUyF9cSaw) or [paper](https://arxiv.org/abs/1801.00862)) — so not perfect million-qubit devices that are needed to run the famous Shor’s or Grover’s algorithms, but rather several-qubit prototypes. \Yogi{Should I shrink it to ref?}\\ \MS{Or a footnote, TBH I'm not sure what will work better, but we can decide on this later. Probably a ref I guess.}

    Some of the main disadvantages of NISQ devices are:
    \begin{itemize}
        \item There’s a lot of noise — e.g. every time you apply a gate, there’s some substantial chance (e.g. 0.1\%) that you’ll actually apply a different gate. And this is just one of many flavours of noise you can get.
        \item The qubits don’t live for too long — after some time you can be pretty confident that whatever information was stored in your system, it’s lost. So the number of operations you can perform in this time is limited. 
        \item You don’t have too many qubits — right now (late 2019) the biggest chips have around 50. Also, there might be some restrictions on which qubits can interact with each other.

    \end{itemize}
    
    This translates to a pretty clear set of restrictions on your quantum circuit:
    
    \begin{itemize}
        \item You can use only N operations per qubit (so called "circuit depth")
        \item You can’t assume everything will go according to plan and there will be no errors along the way. Even if there are errors, you should still get a reasonable (though not perfect) answer. We call this "robustness".
        \item Obviously, you can’t use more qubits than you have.
    \end{itemize}

    So why exactly VQE is a sensible proposition for NISQ devices? \\

    \begin{itemize}
        \item It’s pretty flexible when it comes to the circuit depth, so you can make some tradeoffs. You can use a pretty simple ansatz if you want to keep your circuit very shallow. But once you have a machine which allows you for a deeper circuit — you can use more sophisticated ansatzes and your performance might increase as a result.
        \item VQE has been shown to be somewhat resistant to noise — i.e. even in the presence of noise (up to some levels) it gives you the correct results. Some even claim that a pinch of noise might help with the optimization process, because it helps to escape local minima.
        \item There are some practical problems that do not require a lot of qubits. One example can be nitrogen fixation - an important industrial process  (Honestly, it's not directly about VQE, but you can read details in [this paper](http://arxiv.org/abs/1605.03590)).
    \end{itemize}



 \Yogi{Do you want this here?}
\MS{Not really, Deleted it. }
\MS{TODO add a link to some nice VQE implementation from old screening tasks. }

\end{document}

==> Previous_Sections/deleted.tex <==
% deleted table of contents

\begin{enumerate}
\item\protect\hyperlink{what-does-vqe-even-do}{What does VQE even do?}
\item\protect\hyperlink{why-do-we-care}{Why do we care?}
\item\protect\hyperlink{the-variational-principle}{The variational principle}
\item\protect\hyperlink{what-the-hell-is-an-ansatz}{What the hell is an ``ansatz''?}
\item \protect\hyperlink{what-does-the-circuit-look-like}{What does the
  circuit look like?}
\item\protect\hyperlink{hybrid-approach}{What's this hybrid approach?}
\item\protect\hyperlink{why-is-this-appropriate-for-nisq-devices}{Why is it
  appropriate for NISQ?}
\item \protect\hyperlink{example}{Example}
\end{enumerate}

If you're not familiar with the term, NISQ stands for ``Noisy Intermediate-Scale Quantum,'' so roughly speaking means near-term quantum devices \footnote{Near-term as for 2018}.



Table of contents:
\begin{enumerate}
    \item \hyperlink{combinatorial-optimization-problems}{Combinatorial optimization problems}
    \item \hyperlink{qaoa-introduction}{Introduction to QAOA}
    \item \hyperlink{background-aqc}{Background --- Adiabatic Quantum Computing (AQC)}
    \item \hyperlink{background-quantum-mechanics}{Background --- Quantum Mechanics}
    \item \hyperlink{qaoa-revisited}{QAOA revisited}
    \item \hyperlink{what-does-the-circuit-look-like}{What does the circuit look like}
    \item \hyperlink{why-is-it-appropriate-for-nisq}{Why it's appropriate for NISQ}
    \item \hyperlink{relation-to-vqe}{Relation to VQE}
\end{enumerate}








==> sections/style.tex <==
% some style notes, for the sake of consistency:
%  (I'm writing these down because they were extremely inconsistent at the beginning, and I went through and edited all the posts to adhere to these. -Laura)

% em dashes are done without spaces and with 3 dashes. (I believe this is the common/correct way to do it?) Like this:
%
% She was going to work on the project---until she got sick

% footnotes are after period/comma

% use \tightlist for all lists, both ordered and unordered (unless list items are multiline, have symbols, or otherwise makes it easier to read if they are separated.)
% (this one I didn't go through and edit EVERYTHING, just when I noticed it looked weird.)

